Preference Optimization for Reasoning with Pseudo Feedback

Preference optimization techniques, such as Direct Preference Optimization (DPO), are frequently employed to enhance the reasoning capabilities of large language models (LLMs) in domains like mathematical reasoning and coding, typically following supervised fine-tuning. These methods rely on high-quality labels for reasoning tasks to generate preference pairs; however, the availability of reasoning datasets with human-verified labels is limited. In this study, we introduce a novel approach to generate pseudo feedback for reasoning tasks by framing the labeling of solutions to reason problems as an evaluation against associated test cases. We explore two forms of pseudo feedback based on test cases: one generated by frontier LLMs and the other by extending self-consistency to multi-test-case. We conduct experiments on both mathematical reasoning and coding tasks using pseudo feedback for preference optimization, and observe improvements across both tasks. Specifically, using Mathstral-7B as our base model, we improve MATH results from 58.3 to 68.6, surpassing both NuminaMath-72B and GPT-4-Turbo-1106-preview. In GSM8K and College Math, our scores increase from 85.6 to 90.3 and from 34.3 to 42.3, respectively. Building on Deepseek-coder-7B-v1.5, we achieve a score of 24.6 on LiveCodeBench (from 21.1), surpassing Claude-3-Haiku.

==> depreciated/framework_depreciated.tex <==
\section{Approach}
\label{framework}



\subsection{Problem Formulation}

% Given a set of challenging prompts $\mathcal{X}=\{x_0,x_1,\cdots,x_N\}$, taking $x_i$ as example, the goal is to synthesize a set of solutions $y_{i,j}$ as well as it outcome feedback $r_{i,j}$, where $j$ indicates the $j$-th solution as well as its outcome feedback.

Given an arbitrary prompt $x\in\mathcal{X}$, we can sample multiple solutions $y_i$ from the current policy model $\pi_\theta$. The goal is to obtain the corresponding feedback $r_i$ of $y_i$, so that the policy model is able to be improved through Direct Preference Optimization (DPO)~\citep{dpo}:
\begin{equation}
\label{eqn:dpo}
    \mathcal{L}_{\text{DPO}}(\pi_\theta; \pi_{\text{ref}}; \mathcal{X}) = -\mathbb{E}_{x\in\mathcal{X}, y_i, y_j\sim\pi_\theta(\cdot|x)} 
    \left[ \log \sigma \left( 
        \beta \log \frac{\pi_\theta(y_i | x)}{\pi_{\text{ref}}(y_i | x)}-\beta\log\frac{\pi_\theta(y_j | x)}{\pi_{\text{ref}}(y_j | x)}
    \right) \right] ,
\end{equation}
where $\pi_{\text{ref}}$ is the reference model, $y_i$ is the chosen solution with positive feedback, and $y_j$ is rejected due to a worse feedback. $\beta$ is the hyper-parameter controlling the distance between $\pi_\theta$ and $\pi_{\text{ref}}$.

In this paper, we develop different strategies for mathematical reasoning and code generation according to the task attributes. For mathematical reasoning, the outcome feedback is the equivalence between the predicted answer and the answer label, \ie~$r_{i}\in \{0,1\}$. For programming, supposing that we have a set of test cases $\mathcal{T}=\{\tuple{I_{1},O_{1}},\tuple{I_{2},O_{2}},\cdots,\tuple{I_{T},O_{T}}\}$, where $\tuple{I_{j},O_{j}}$ indicates the $j$-th test input-output pair for prompt $x$, the execution feedback is defined as the averaged pass rate on $\mathcal{T}$ with the predicted program, \ie~
\begin{equation}
    r_{i}=\frac{1}{T}(\sum_{j=1}^T \mathbbm{1}(\mathrm{exec}(y_{i}, I_{j})=O_{j})),
\end{equation}
where $\mathrm{exec}(y, I)$ refers to the operation by running the predicted program contained in $y$ on the given test case inputs $I$, and parsing the corresponding outputs.



\subsection{Learning from Feedback}

% By taking the solutions with outcome feedback, we can optimize the model by  Direct Preference Optimization (DPO). Specifically, we can construct a preference dataset as follow:
By taking the complete solutions with outcome feedback, we can optimize the model through DPO according to Equation~\ref{eqn:dpo}. Specifically, we can construct the preference dataset as follow:
% ,x\in\mathcal{X},y_i,y_j\sim\pi_\theta(\cdot|x)
\begin{equation}
    \mathcal{D}_o=\{(x,y_{i},y_{j})|r_{i} \ge \epsilon, r_{i} - r_{j} > \sigma\},
\end{equation}
where $y_{i}$ and $y_{j}$ are the chosen and rejected solutions \wrt prompt $x$, $\epsilon$ and $\sigma$ are two hyper-parameters controlling the quality lower-bound of positive samples and the margin, respectively.

Besides, some of recent studies demonstrate that the outcome feedback can be used to estimate the expected returns of intermediate reasoning steps, which can help the model produce better reasoning trajectory. Motivated from this, we also construct the process preference dataset.
Following \citet{jiao2023pdpo}, given the solution prefix $\tilde{y}$, we employ the same policy model to sample $K$ completions following $\tilde{y}$, and treat the averaged outcome feedback $\tilde{r}$ of the completions as the expected returns of $\tilde{y}$. After that, the process preference dataset can be defined as:
\begin{equation}
    \mathcal{D}_p=\{(x,\tilde{y}_{i},\tilde{y}_{j})|\tilde{r}_{i} \ge \epsilon, \tilde{r}_{i} - \tilde{r}_{j} > \sigma\},
\end{equation}
where $\tilde{y}_{i}$ and $\tilde{y}_{j}$ are randomly sampled prefixes belonging to some complete solutions.

During training, we combine both the process-preference dataset and the outcome based one together. We also include the NLL loss on the chosen solutions in each forward step.

\input{iclr2025/figures/code-sc}


\subsection{Self-Consistency-based Pseudo Label Generation}
\label{sec:code-dpo}

In this section, we will introduce how to synthesize the pseudo feedback based on self-consistency. 
For mathematical reasoning, the pseudo feedback is defined as the equivalence between the predicted answer and the pseudo label obtain via self-consistency.

% Employing self-consistency to construct pseudo outcome feedback can be intuitive. 
% Learning from reliable feedback for continuous improvements have been widely studied~\citep{openai-verify,cobbe2021training}. Despite the different learning strategies, the ultimate challenge is how could we obtain sustainable and reliable feedback, with both development of the capability of model and the complexity of environment.

% Some recent studies have attempted to employ self-consistency to produce pseudo feedback~\citep{huang2022large}. 
% Yet, the efforts have been put on neither stronger models to solve more challenging problems, nor tasks where the consistency is difficult to be determined.
% Yet, the efforts have been in an early stage, without touch on stronger models, more challenging problems, as well as tasks where the consistency is difficult to be measured.
% In this paper, for mathematical reasoning, we employ \llama-base and \mathstral~for experiments, where the pseudo feedback is defined as the equivalence between predicted answer and the pseudo label obtained via self-consistency.
% We simply sample multiple solutions for each prompt, and treat the answer candidate with the highest frequency as the pseudo label to obtain the outcome feedback. 

For code generation, since self-consistency cannot be directly applied to programs, we thus propose a novel test case-based strategy.
Specifically, given $K$ predicted programs for the same prompt, as well as $T$ groups of test case  inputs $\{I_0,I_1,\cdots,I_T\}$, we can run these programs on each group of inputs to obtain the corresponding outputs. As a consequence, for each group of inputs $I_i$, we have $K$ groups of outputs $\mathcal{O}_i=\{O_{i,j}|\,0\le j < K\}$. We then perform self-consistency along the program dimension to annotate the pseudo outputs for each group of inputs. Finally, we could obtain series of pseudo test cases: $\tilde{\mathcal{T}}=\{\tuple{I_{0},\tilde{O}_{0}},\tuple{I_{1},\tilde{O}_{1}},\cdots,\tuple{I_{T},\tilde{O}_{T}}\}$, where $\tilde{O}_{i}$ is the group of outputs with highest frequency among $\mathcal{O}_i$. Figure~\ref{fig:code-framework} shows a simplified case for this process.

Another challenge we face is the inability to obtain standard test cases all the time, even when only inputs are required. For instance, most test cases of the problems from Codeforces~\footnote{\href{https://codeforces.com/}{https://codeforces.com/}} are hidden to avoid being hacked. \citet{alpha-code} addressed this issue by training a specialized model for test case inputs generation. Inspired by this approach, we query general-purpose large language models, such as GPT-4o and Mistral-Large-2, to generate the test case inputs. This method effectively enables a fully synthetic approach for constructing pseudo-feedback.\footnote{Though we employed larger model for test case inputs generation, we argue that it is much easier than code generation, since we would always provide all available information to the model for assistance, including function head, example input-output pairs, and the notes about testing limits.}.

In addition, we incorporate pseudo feedback from a teacher model. For mathematical reasoning tasks, we simply use the predicted answer from the teacher model as a pseudo label to synthesize feedback, as illustrated in the upper right of Figure~\ref{fig:framework}. A similar strategy can be applied to code generation, where the outputs of teacher-generated programs are treated as pseudo outputs for the test cases\footnote{We did not employ teacher-generated pseudo feedback in code generation since we find the one constructed from self-generated solutions already works well.}. 
% However, we have not yet explored the use of teacher-generated pseudo-feedback in the code generation domain.

\input{iclr2025/figures/framework}

\subsection{Training Pipeline}

Starting with a base policy model, we first apply supervised fine-tuning (SFT) to enable the model to acquire foundational knowledge from the teacher model. 
To achieve further improvements, we introduce pseudo-feedback into an iterative training process. Figure~\ref{fig:framework} illustrates the process for a single iteration. 
In each round, we collect multiple solutions for each prompt generated by the current best policy model, construct pseudo-feedback, and then perform DPO training. 
The prompt set used between iterations can remain the same or vary, depending on the size of collected dataset.



==> iclr2025/tables/math_full.tex <==
\begin{table}[t]
\centering
% \vskip 0.05in
\renewcommand{\arraystretch}{1.2}
\setlength{\tabcolsep}{4.0mm}{
\scalebox{0.9}{
\begin{tabular}{l|ccc}
\toprule
                                & MATH          & GSM8K         & MWPBench  \\ \hline
% Deepseek-Coder-v2-Lite-Instruct & 61.8          & 86.4          & --- \\
% Qwen2-Math-7B-Instruct          & 75.1          & 89.9          & ---   \\
% NuminaMath-72B-CoT              & 66.7          & 90.8          & ---   \\ \hline
GPT-4o-2024-0512$^\dag$         & 76.6          & ---           & --- \\
GPT-4-Turbo-2024-0409$^\dag$    & 73.4          & ---           & --- \\
GPT-4-Turbo-1106-preview$^\dag$ & 64.3          & ---           & --- \\
GPT-4-0613$^\ddag$              & 51.8          & 92.9          & 52.0 \\ \hline
Qwen2-Math-7B-Instruct          & 75.1          & 89.9          & 62.1   \\
NuminaMath-72B-CoT              & 66.7          & 90.8          & 57.8   \\ 
Llama-3.1-8B-Instruct           & 49.0          & 85.1          & 48.5 \\
Llama-3.1-70B-Instruct          & 65.7          & 94.1          & 60.5      \\\hline
Llama-3.1-8B-base               &               &               &        \\
~~w/ SFT (M.S.-500k)            & 52.8          & 85.1          & 49.2   \\
~~~~w/ DPO (M.S.-500k)          & 53.1          & 86.0          & 51.3       \\ 
~~~~w/ pDPO (M.S.-500k)         & 54.3          & 86.6          & 52.1        \\
~~~~~~w/ pDPO (Numina-S.C. 160k)     & 54.8 & 87.6 & 52.6      \\ 
~~~~~~~~w/ pDPO (Numina-S.C. 320k)& 55.7 & \textbf{88.8}    & \textbf{53.3} \\ 
~~~~~~~~~~w/ pDPO (Numina-S.C. 480k)& \textbf{56.2} & 88.7      & 53.2  \\\hline
Mathstral-7B-v0.1               & 56.6          & 82.8          & 49.8   \\
~~w/ SFT (M.S.-500k)            & 61.5          & 86.9          & 54.1       \\
~~~~w/ DPO (M.S.-500k)          & 62.2          & 88.5          & 56.3       \\
~~~~w/ pDPO (M.S.-500k)         & 65.6          & 89.8          & 59.0       \\
~~~~~~w/ pDPO (M.S.-300k-S.C., Iter. 0) & 66.7 & \textbf{90.8} & 60.0      \\
~~~~~~~~w/ pDPO (M.S.-300k-S.C., Iter. 1) & \textbf{67.5} & 90.3 & \textbf{60.1}      \\
\bottomrule
\end{tabular}
}}
\caption{Overall results on mathematical reasoning benchmarks. The indentation across different levels represents the corresponding model is initialized from the parent-level. \textit{M.S.} refers to the short of \textit{MathScale}, and \textit{S.C.} means \textit{Self-Consistency}.}
\label{tab:math-full}
\end{table}

==> iclr2025/tables/math_v2.0.tex <==
\begin{table}[t]
\centering
% \vskip 0.05in
\renewcommand{\arraystretch}{1.2}
\setlength{\tabcolsep}{3.2mm}{
\scalebox{0.85}{
\begin{tabular}{l|ccccc}
\toprule
                                & MATH          & GSM8K         & Gaokao 2023   & Colledge Math & MWPBench  \\ \hline
GPT-4o-2024-0512$^\dag$         & 76.6          & 95.7          & ---           & 31.54         & --- \\
GPT-4-Turbo-2024-0409$^\dag$    & 73.4          & ---           & ---           & ---           & --- \\
GPT-4-Turbo-1106-preview$^\dag$ & 64.3          & ---           & ---           & ---           & --- \\
GPT-4-0613$^\ddag$              & 51.8          & 92.9          & 24.4          &               & 52.0 \\ \hline
% Deepseek-Coder-v2-Lite-Instruct & 61.8          & 86.4          &               &               & --- \\
% Deekseek-Math-7B-RL             & 52.4          & 88.2          &               & 37.5          &       \\ % I prefer to temperally remove this model since it requires different evaluation strategy
Qwen2-Math-7B-Instruct          & 75.1          & 89.9          & 43.3          & 30.6          & 62.1   \\
NuminaMath-72B-CoT              & 66.7          & 90.8          & 50.0          & 27.8          & 57.8   \\ 
% Llama-3.1-8B-Instruct           & 47.2          & 76.6          &               & 33.8          &          \\
Llama-3.1-8B-Instruct           & 49.0          & 85.1          & 33.3          & 25.3          & 48.5 \\
Llama-3.1-70B-Instruct          & 65.7          & 94.1          & 43.3          & 31.1          & 60.5      \\\hline
Llama-3.1-8B-base               &               &               &               &               &        \\
% ~~w/ SFT (M.S.-500k)            & 52.8          & 85.1          &               &               & 49.2   \\
% ~~~~w/ DPO (M.S.-500k)          & 53.1          & 86.0          &               &               & 51.3       \\ 
% ~~~~w/ pDPO (M.S.-500k)         & 54.3          & 86.6          &               &               & 52.1        \\
% ~~~~~~w/ pDPO (Numina-S.C. 160k)     & 54.8     & 87.6          &               &               & 52.6      \\ 
% ~~~~~~~~w/ pDPO (Numina-S.C. 320k)& 55.7 & \textbf{88.8}        &               &               & \textbf{53.3} \\ 
% ~~~~~~~~~~w/ pDPO (Numina-S.C. 480k)& \textbf{56.2} & 88.7      &               &               & 53.2  \\\hline
~~w/ SFT-4o                       & 52.8          & 85.1          & 30.0          & 26.8          & 49.2   \\
~~~~w/ \ariat~Iter. 0         & 54.3          & 86.6          & \textbf{36.7} & 28.3          & 52.1        \\
~~~~w/ \arias~Iter. 1            & 54.8          & 87.6          & 33.3          & 28.7          & 52.6      \\ 
~~~~w/ \arias~Iter. 2            & 55.7          & \textbf{88.8} & \textbf{36.7} & \textbf{29.3} & \textbf{53.3} \\ 
~~~~w/ \arias~Iter. 3            & \textbf{56.2} & 88.7          & \textbf{36.7} & 28.5          & 53.2  \\\hline
Mathstral-7B-v0.1               & 56.6          & 82.8          & 30.0          & 25.8          & 49.8   \\
~~w/ SFT-4o            & 61.5          & 86.9          & 36.7          & 28.4          & 54.1       \\
% ~~~~w/ DPO (M.S.-500k)          & 62.2          & 88.5          &               &               & 56.3       \\
~~~~w/ \ariat~Iter. 0         & 65.6          & 89.8          & 43.3          & 29.9          & 59.0       \\
~~~~w/ \arias~Iter. 1            & 66.7          & \textbf{90.8} & \textbf{50.0} & 30.7          & 60.0      \\
~~~~w/ \arias~Iter. 2            & \textbf{67.5} & 90.3          & \textbf{50.0} & \textbf{30.8} & \textbf{60.1}      \\
\bottomrule
\end{tabular}
}}
\caption{Overall results on mathematical reasoning benchmarks. \textit{4o} refers to the training phase employing the pseudo feedback from teacher model (GPT-4o), while \textit{Self} indicates the phase using pseudo feedback constructed from self-generated solutions. $^\dag$: Results are from \citet{persona-hub}. $^\ddag$: Results are from \citet{tang2024mathscale}.}
\label{tab:math}
\end{table}
